Lossless preprocessing of floating point data to enhance compression

Data compression algorithms typically rely on identifying repeated sequences of symbols from the original data to provide a compact representation of the same information, while maintaining the ability to recover the original data from the compressed sequence. Using data transformations prior to the compression process has the potential to enhance the compression capabilities, being lossless as long as the transformation is invertible. Floating point data presents unique challenges to generate invertible transformations with high compression potential. This paper identifies key conditions for basic operations of floating point data that guarantee lossless transformations. Then, we show four methods that make use of these observations to deliver lossless compression of real datasets, where we improve compression rates up to 40 %.

==> sections/Bibliography.tex <==
\begin{thebibliography}{8}
	\bibitem{additionmethod}
	F. Taurone \textit{et al.}, ``Change a Bit to save Bytes: Compression for Floating Point Time-Series Data," accepted to IEEE International Conference on Communications (ICC), 2023, Available online: \url{	arXiv:2303.04478}.

	\bibitem{GD_Greedy}
	A. Hurst \textit{et al.}, `"GreedyGD : Enhanced Generalized Deduplication for Direct Analytics in IoT, submitted to IEEE Transactions on Industrial Informatics, 2022, Available online: \url{http://arxiv.org/abs/2304.07240}.

	\bibitem{IEEE754}
	IEEE Std 754-2019 IEEE Standard for Floating-Point Arithmetic.

	\bibitem{zlib}
	Zlib compressor \url{https://www.zlib.net/}.

	\bibitem{FPHandbook}
	J.-M. Muller \textit{et al.}, ``Handbook of Floating-Point Arithmetic," 2010.

	\bibitem{FProunding}
	Mark D. Hill, ``Notes on floating point arithmetic, part of course CS/ECE 354 at University of Wisconsin," \url{https://tinyurl.com/mvzcyc3x}.

	\bibitem{TaxiDataset}
	``Taxi trips dataset" 2022, \url{https://tinyurl.com/4rypurjp}.

	\bibitem{UciDataset}
	H. Kaya \textit{et al.}, ``Gas turbine CO and NOx emission dataset,", 2019. \url{https://tinyurl.com/2ubk63ra}.

	%\bibitem{GD_Bounds}
	%R. Vestergaard, Q. Zhang, D. E. Lucani, ``Generalized Deduplication: Bounds, Convergence, and Asymptotic Properties," IEEE Global Communications Conference (GLOBECOM), Waikoloa, HI, USA, 2019, pp. 1-6.

	\bibitem{GD_RandomAccess}
	R. Vestergaard \textit{et al.}, ``A Randomly Accessible Lossless Compression Scheme for Time-Series Data," IEEE INFOCOM 2020.

	\bibitem{GD_analytics}
	A. Hurst \textit{et al.}, ``GLEAN: Generalized-Deduplication-Enabled Approximate Edge Analytics," IEEE Internet of Things Journal 2023.

	\bibitem{dct}
	Batal Iyad \textit{et al.},  ``A Supervised Time Series Feature Extraction Technique Using DCT and DWT", ICMLA, 2009.
	
	\bibitem{infoPreprocessing}
	M. Klöwer \textit{et al.}, ``Compressing atmospheric data into its real information content", Nature, 2021.

\begin{comment}
	\bibitem{ref_lncs1}
	Author, F., Author, S.: Title of a proceedings paper. In: Editor,
	F., Editor, S. (eds.) CONFERENCE 2016, LNCS, vol. 9999, pp. 1--13.
	Springer, Heidelberg (2016). \doi{10.10007/1234567890}

	\bibitem{ref_book1}
	Author, F., Author, S., Author, T.: Book title. 2nd edn. Publisher,
	Location (1999)

	\bibitem{ref_proc1}
	Author, A.-B.: Contribution title. In: 9th International Proceedings
	on Proceedings, pp. 1--2. Publisher, Location (2010)

	\bibitem{ref_url1}
	LNCS Homepage, \url{http://www.springer.com/lncs}. Last accessed 4
	Oct 2017
\end{comment}

\end{thebibliography}

